Mirror Mirror on the Wall, Have I Forgotten it All? A New Framework for Evaluating Machine Unlearning

Machine unlearning methods take a model trained on a dataset and a forget set, then attempt to produce a model as if it had only been trained on the examples not in the forget set. We empirically show that an adversary is able to distinguish between a mirror model (a control model produced by retraining without the data to forget) and a model produced by an unlearning method across representative unlearning methods from the literature. We build distinguishing algorithms based on evaluation scores in the literature (i.e. membership inference scores) and Kullback-Leibler divergence. We propose a strong formal definition for machine unlearning called computational unlearning. Computational unlearning is defined as the inability for an adversary to distinguish between a mirror model and a model produced by an unlearning method. If the adversary cannot guess better than random (except with negligible probability), then we say that an unlearning method achieves computational unlearning. Our computational unlearning definition provides theoretical structure to prove unlearning feasibility results. For example, our computational unlearning definition immediately implies that there are no deterministic computational unlearning methods for entropic learning algorithms. We also explore the relationship between differential privacy (DP)-based unlearning methods and computational unlearning, showing that DP-based approaches can satisfy computational unlearning at the cost of an extreme utility collapse. These results demonstrate that current methodology in the literature fundamentally falls short of achieving computational unlearning. We conclude by identifying several open questions for future work.

==> sections/LinRegUnlearning.tex <==
\section{Perfect Unlearning for Linear Regression}
\label{sec:perfect-lin-reg}

We now demonstrate a method of computational unlearning for least-squares linear regression models. Recall that linear regression is defined for data matrix $\mathbf{X} \in \mathbb{R}^{m \times n}$ with associated observed outputs $y \in \mathbb{R}^m$. For convenience, let $\mathbf{x}_i \in \mathbb{R}^n$ denote the $i$-th row of $\mathbf{X}$, and let $y_i$ denote the $i$-th component of $\mathbf{y}$. We want to find a coefficient vector $\mathbf{a} \in \mathbb{R}^n$ s.t.

$$\mathbf{a} = \argmin_{\mathbf{v} \in \mathbb{R}^n}{\|\mathbf{Xv} - \mathbf{y}\|^2}$$

Recall then that the solution $\mathbf{a}$ is given by 

$$\mathbf{a} = (\mathbf{X}^T\mathbf{X})^{-1}\mathbf{X}^T\mathbf{y}$$

Now, assume without loss of generality that we want to forget $\left(\mathbf{x}_m, y_m\right)$. Our resulting retain set can then be written as follows.

$$
\mathbf{X}_R = \left(\begin{matrix}
    \mathbf{x}_1 & \rightarrow \\
    \mathbf{x}_2 & \rightarrow \\
    \vdots \\
    \mathbf{x}_{m - 1} & \rightarrow
\end{matrix}\right) \in \mathbb{R}^{m \times n} , \ 
\mathbf{y}_R = \left(\begin{matrix}
    y_1 \\
    y_2 \\
    \vdots \\
    y_{m - 1}
\end{matrix}\right) \in \mathbb{R}^m
$$

Observe that we can create a ``forgetting transform'' matrix $\mathbf{U}$ to map $\mathbf{X}$ to $\mathbf{X}_R$ and $\mathbf{y}$ to $\mathbf{y}_R$, where 

$$
\mathbf{U} = \left(\begin{matrix}
    \mathbf{I}_{m - 1} & \mathbf{0}
\end{matrix}
\right) \in \mathbb{R}^{(m - 1) \times m}
$$ \phil{Need to figure out block matrices}

Now, recall that the least squares solution for $\mathbf{X}_R$, $\mathbf{y}_R$ can is given by $\mathbf{a}_R = \left(\mathbf{X}_R^T\mathbf{X}_R\right)^{-1}\mathbf{X}_R^T\mathbf{y}_R$. We can rewrite this as follows:

$$
\left(\mathbf{X}_R^T\mathbf{X}_R\right)^{-1}\mathbf{X}_R^T\mathbf{y}_R = \left((\mathbf{U}\mathbf{X})^T(\mathbf{U}\mathbf{X})\right)^{-1}(\mathbf{U}\mathbf{X})^T(\mathbf{U}\mathbf{y}) = \left(\mathbf{X}^T\mathbf{U}^T\mathbf{U}\mathbf{X}\right)^{-1}\mathbf{X}^T\mathbf{U}^T\mathbf{U}\mathbf{y}
$$

Now, observe the following
$$
\mathbf{U}^T\mathbf{U}\mathbf{X} = \mathbf{U}^T\mathbf{X}_R = \left(\begin{matrix}
    \mathbf{x}_1 & \rightarrow \\
    \mathbf{x}_2 & \rightarrow \\
    \vdots \\
    \mathbf{x}_{m - 1} & \rightarrow \\
    \mathbf{0} & \rightarrow
\end{matrix}\right) , \
\mathbf{U}^T\mathbf{U}\mathbf{y} = \mathbf{U}^T\mathbf{y}_R = \left(\begin{matrix}
    y_1 \\
    y_2 \\
    \vdots \\
    y_{m - 1} \\
    0
\end{matrix}\right)
$$
$$
\Rightarrow \mathbf{X}^T\left(\begin{matrix}
    \mathbf{x}_1 & \rightarrow \\
    \mathbf{x}_2 & \rightarrow \\
    \vdots \\
    \mathbf{x}_{m - 1} & \rightarrow \\
    \mathbf{0} & \rightarrow
\end{matrix}\right) = \mathbf{X}^T\mathbf{X} - \mathbf{x}_m\mathbf{x}_m^T , \
\mathbf{X}^T\left(\begin{matrix}
    y_1 \\
    y_2 \\
    \vdots \\
    y_{m - 1} \\
    0
\end{matrix}\right) = \mathbf{X}^T\mathbf{y} - y_m\mathbf{x}_m
$$
Thus, we can rewrite the solution for $\mathbf{a}_R$ as follows

\begin{align*}
    \Rightarrow \left(\mathbf{X}^T\mathbf{U}^T\mathbf{U}\mathbf{X}\right)^{-1}\mathbf{X}^T\mathbf{U}^T\mathbf{U}\mathbf{y} &= \left(\mathbf{X}^T\mathbf{X} - \mathbf{x}_m\mathbf{x}_m^T\right)^{-1}\left(\mathbf{X}^T\mathbf{y} - y_m\mathbf{x}_m\right) \\
    &= \left(\mathbf{X}^T\mathbf{X} - \mathbf{x}_m\mathbf{x}_m^T\right)^{-1}\left(\mathbf{X}^T\mathbf{y}\right) - \left(\mathbf{X}^T\mathbf{X} - \mathbf{x}_m\mathbf{x}_m^T\right)^{-1}\left(y_m\mathbf{x}_m\right)
\end{align*}


Now, using the Sherman-Morrison formula \phil{cite this}, we can calculate $\left(\mathbf{X}^T\mathbf{X} - \mathbf{x}_m\mathbf{x}_m^T\right)^{-1}$ cheaply, and the remaining calculations are simple matrix multiplications. Thus, we can compute the unlearned model coefficients $\mathbf{a}_R$ quicker than retraining the model from scratch \phil{Should provide an actual analysis; forgot the runtime of the Sherman-Morrison algo}. Since the formula was derived directly from the retrained model, it is guaranteed to match it \emph{exactly}, thus making this a clear example of computational unlearning. 


==> sections/Shortcoming-Examples.tex <==
\ifdefined\oakland
\begin{figure*}[t]
    \centering
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \includegraphics[width=\textwidth]{mse_classwise_cifar.png}
    %     \caption{Unaltered image.}
    % \end{subfigure}\hfil
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \includegraphics[width=\textwidth]{mse_classwise_cifar.png}
    %     \caption{Noised image.}
    % \end{subfigure}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_1.png}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_2.png}\\ \vspace{.75em}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_0.png}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_3.png} \\ \vspace{.75em}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_117.png}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_10.png}
    \caption{Examples of recovering forgotten behavior on CIFAR-10 \autocite{2009Krizhevsky_cifar}. The unlearned model (produced using amnesiac unlearning from \autocite{2020Graves_Amnesiac}) performs poorly on the unaltered images but well on the perturbed image. Perturbations were done using Pixle \autocite{2022Pomponi_Pixle}, a black-box adversarial technique.}
    \label{fig:mia-fails}
\end{figure*}
\fi
\ifdefined\preprint
\begin{figure*}
    \centering
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \includegraphics[width=\textwidth]{mse_classwise_cifar.png}
    %     \caption{Unaltered image.}
    % \end{subfigure}\hfil
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \includegraphics[width=\textwidth]{mse_classwise_cifar.png}
    %     \caption{Noised image.}
    % \end{subfigure}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_1.png}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_2.png}\\ \vspace{.75em}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_0.png}
    \includegraphics[width=.45\textwidth]{mia-counterexamples/img_3.png} %\\ \vspace{.75em}
    %\includegraphics[width=.45\textwidth]{mia-counterexamples/img_117.png}
    %\includegraphics[width=.45\textwidth]{mia-counterexamples/img_10.png}
    \caption{Examples of recovering forgotten behavior on CIFAR-10 \autocite{2009Krizhevsky_cifar}. The unlearned model (produced using amnesiac unlearning from \autocite{2020Graves_Amnesiac}) performs poorly on the unaltered images but well on the perturbed image. Perturbations were done using Pixle \autocite{2022Pomponi_Pixle}, a black-box adversarial technique.}
    \label{fig:mia-fails}
\end{figure*}
\fi


==> sections/UnlearningTable.tex <==
% \brennon{What is this table doing for us at this point? We probably want to sumamrize a different way.}

% \begin{table*}[t]
% \begin{center}
% \begin{threeparttable}
% \begin{tabular}{rccccccc} \toprule
%     Name & Category & Randomized & DP & Setting 1 & Setting 2 & Setting 3 & CU Candidate\tnote{1} \\ 
%     \midrule
%     Negative Gradient & Heuristic & \xmark & \xmark & \xmark \\
%     SSD \autocite{2020bourtoule_machine} & Heuristic & \xmark & \xmark & \xmark \\
%     Amnesiac \autocite{2020Graves_Amnesiac} & Heuristic & \xmark & \xmark & \xmark \\
%     Bad Teacher \autocite{2023Chundawat_bad_teaching} & Heuristic & \cmark & \xmark & \xmark \\
%     Scrubbing \autocite{2020Golatkar_Eternal_Sunshine} & Approximate & \cmark & \xmark & IDK yet\\ 
%     DP-SGD \autocite{2016Abadi_DP_SGD} & Approximate & \cmark & \cmark & \cmark \\ 
%     Laplacian Mechanism\footnote{\brennon{See example 3.2 from \autocite{2014dwork_dp}}} & Approximate & \cmark & \cmark & \cmark \\ 
%     Ullah et. al \autocite{2021Ullah_TV_Stability} & Approximate? & \cmark & \cmark & \cmark \\
%     \bottomrule
% \end{tabular}
% \begin{tablenotes}
%     \item [1] CU candidate: shorthand for an algorithm that is a candidate for computational unlearning (see Definition \ref{def:computational-unlearning}). A candidate algorithm must be randomized and pass our attacks in Setting 1, 2, and 3.
% \end{tablenotes}
% \vspace{-9em}
% \caption{Summary of existing unlearning methods in context of computational unlearning. \phil{expand as more are added}}
% \label{tbl:summary}
% \end{threeparttable}
% \end{center}
% \end{table*}

